Constraining the evolution of red supergiants with the integrated light of star clusters

The integrated properties of young star clusters are subject to large cluster-to-cluster variations because they depend directly on small numbers of bright stars. At ages at which red supergiants are expected to exist, these luminous but rare stars can be blamed for most of the variations. If unresolved clusters are to be used to constrain red supergiant models, methods must be developed that take these stochastic fluctuations into account. We discuss prospects and open issues in this field, based on recent work on high mass clusters in M82, and on first experiments towards a Bayesian study of cluster populations.

==> abstract <==
Title: Constraining the evolution of red supergiants with the
 integrated light of star clusters
Authors: Ariane Lan\c{c}on and  Morgan Fouesneau  
 (Observatoire de Strasbourg, UMR 7550, France)
Comments: 6 pages, 1 figure (4 postscript inserts), uses asp2006_hotcool.sty. 
 To be published in "Hot and Cool: Bridging Gaps in Massive Star Evolution",
 ed. C. Leitherer, Ph. D. Bennett, P. W. Morris, J. Th. van Loon (San
 Francisco: ASP)

The integrated properties of young star clusters are subject to
large cluster-to-cluster variations because they depend directly on
small numbers of bright stars. At ages at which red supergiants are
expected to exist, these luminous but rare stars can be blamed
for most of the variations. If unresolved clusters are to be used
to constrain red supergiant models, methods must be developed that
take these stochastic fluctuations into account. We discuss
prospects and open issues in this field, based on recent
work on high mass clusters in M82, and on first experiments
towards a Bayesian study of cluster populations.

